Will This Video Go Viral? Explaining and Predicting the Popularity of Youtube Videos

What makes content go viral? Which videos become popular and why others don't? Such questions have elicited significant attention from both researchers and industry, particularly in the context of online media. A range of models have been recently proposed to explain and predict popularity; however, there is a short supply of practical tools, accessible for regular users, that leverage these theoretical results. HIPie -- an interactive visualization system -- is created to fill this gap, by enabling users to reason about the virality and the popularity of online videos. It retrieves the metadata and the past popularity series of Youtube videos, it employs Hawkes Intensity Process, a state-of-the-art online popularity model for explaining and predicting video popularity, and it presents videos comparatively in a series of interactive plots. This system will help both content consumers and content producers in a range of data-driven inquiries, such as to comparatively analyze videos and channels, to explain and predict future popularity, to identify viral videos, and to estimate response to online promotion.

==> 5-creators.tex <==
%!TEX root = hip-demo.tex

\section*{Authors}

\newcommand\mytextwidth{19.5em} 
\newcommand\myheight{0.09}
\begin{tabular} {ll}
      \parbox[c]{\myheight\textheight}{
          \includegraphics[height=\myheight\textheight]{me}
      } & \parbox[c]{\mytextwidth}{\textbf{Quyu Kong} received his Bachelor of Agronomy at the Zhejiang University in 2015 and Master of Computing (Advanced) degree in Artificial Intelligence at the Australian National University in 2017. His research interests include Information Diffusion Modeling and Machine Learning.} \\
     & \\
     \parbox[c]{\myheight\textheight}{
          \includegraphics[height=\myheight\textheight]{andrei}
      } & \parbox[c]{\mytextwidth}{\textbf{Marian-Andrei Rizoiu} is a Research Fellow with the Australian National University. 
		He employs big social data to develop theoretical models for novel societal phenomena, such as information diffusion in online networks and online popularity modeling and prediction.      
%      His main research interests are Online Information Diffusion, Theoretical Popularity Modeling, Online Privacy, Social Networks, Machine Learning, Data Mining and Big Data \TODO{MAR}{Update this}.
      } \\
      & \\
     \parbox[c]{\myheight\textheight}{
         \includegraphics[height=\myheight\textheight]{siqi}
      } 
      & \parbox[c]{\mytextwidth}{\textbf{Siqi Wu} is a PhD student at the Australian National University. His research focuses on the analysis of user engagement in online media and influential network in social graph.} \\
	& \\
     \parbox[c]{\myheight\textheight}{
          \includegraphics[height=\myheight\textheight]{lexing}
      } 
      & \parbox[c]{\mytextwidth}{\textbf{Lexing Xie} is an Associate Professor in computer science with the College of Engineering and Computer Science in the Australian National University, leading the ANU Computational Media Lab. Her research focuses broadly on innovative use and design of machine learning algorithms and systems, especially on structured and multi-relational graph data.} \\
\end{tabular}



==> fig2-sir-as-two-processes.tex <==
%!TEX root = sir-hawkes.tex

\begin{figure}[tbp]
	\centering
	\includegraphics[width=0.47\textwidth]{two_processes}
	
	\caption{An illustration of SIR as a bivariate Poisson process: the infection process and the recovery processes.
	\emph{(top panel)} Each of the five individuals gets infected at time $t^I_j$ and recovers at $t^R_j$. 
	Each individual $j$ stays infectious for a period $\tau_j$.
	For the equivalence with HawkesN, only new infection times $t^I_j$ are observed, the new recovery times $t^R_j$ are unobserved.
	\emph{(middle panel)} The corresponding size of the infectious population $I(t)$ over time.
	\emph{(lower panel)} The new infection rate $\lambda^I(t)$ and the new recovery rate $\lambda^R(t)$.
	SIR parameters: $N = 5$, $\beta = 2$, $\gamma = 0.5$.
	}
	\label{fig:sir-two-processes}
	\captionmoveup
\end{figure}


==> fig3-markov-states-probs.tex <==
%!TEX root = sir-hawkes.tex

\begin{figure}[tbp]
	\centering
	\includegraphics[width=0.23\textwidth]{markov-chain-states}
	
	\caption{
		Visualization of the space of states of the SIR bivariate Markov Chain $\{s, i\}$.
		$s, i \in \mathbbm{N}$ and $s + i \leq N $, in other words the space of valid states sits under the green line $s+i = N$. 		
		The initial state in an SIR epidemic is always on the \textcolor{ForestGreen}{green line} ($S(0) + I(0) = N$). 
		Given an initial state $\{s = S(0), i = I(0)\}$ (shown by the \textcolor{DarkMagenta}{magenta circle}), the \textcolor{DarkOrange}{orange area} shows the space of reachable states and the \textcolor{gray}{gray area} depicts the \emph{unreachable states}.
		From a state $\{s,i\}$ the system can to $\{s-1,i+1\}$ 
		%with probability $p_{(s-1,i+1),(s,i)}$ 
		(new infection); and to $\{s,i-1\}$ 
		%with probability $p_{(s,i-1),(s,i)}$ 
		(new recovery).
		The absorbing states ($\{s, 0\}$) is shown with a \textcolor{red}{red line}.
	}
	\label{fig:markov-chain}
	\captionmoveup
\end{figure}


==> fig3-stochastic-vs-deterministic-sir.tex <==
%!TEX root = sir-hawkes.tex

\begin{figure}[tbp]
	\centering
	\newcommand\myheight{0.18}
	\subfloat[] {
		\includegraphics[page=1,height=\myheight\textheight]{stochastic-vs-deterministic-sir}
%		\label{subfig:popularity-scale-90}
	}
	\subfloat[] {
		\includegraphics[page=2,height=\myheight\textheight]{stochastic-vs-deterministic-sir}
%		\label{subfig:popularity-scale-120}
	}  \\
	\subfloat[] {
		\includegraphics[page=3,height=\myheight\textheight]{stochastic-vs-deterministic-sir}
%		\label{subfig:popularity-scale-jump}
	}
	\subfloat[] {
		\includegraphics[page=4,height=\myheight\textheight]{stochastic-vs-deterministic-sir}
%		\label{subfig:popularity-scale-jump}
	}
	\caption{ 
		We simulate 100 stochastic SIR realizations using the parameters $N = 1300, I(0) = 300, \beta = 1, \gamma = 0.2$.
		We show the median and the $2.5\%$ and $97.5\%$ percentile and the deterministic evolution simulated with the same parameters.
		We also show an example of stochastic realization.
	}
	\label{fig:stochastic-vs-deterministic-SIR}
\end{figure}
